Backdoor Decontamination Dynamics in LLM Agents

Open-weight LLM agents are vulnerable to backdoors installed during fine-tuning, which may be undetectable if the trigger conditions are never met during testing. Assuming defenders do not know the existing trigger, they cannot unlearn it directly. One decontamination strategy is to install a known backdoor (defensive poisoning) then to unlearn it, hoping that the original unknown backdoor is removed as a side effect. However, this procedure has uncertain outcomes: the original backdoor may persist or be erased or rerouted, among other possibilities. We introduce a framework for studying these dynamics in tool-calling agents, decoupling trigger, response, teacher, and fine-tuning method across systematic experiments on AgentDyn. Across 115 experiments, defensive poisoning alone erases around 56% of original backdoors; subsequent decontamination then drives almost all survivors to erasure, confirming that trigger recognition and malicious execution are behaviorally dissociable. Interestingly, our experiments find that malicious backdoors never persist when using different triggers of the same general type as the defensive backdoor when followed by decontamination via unlearning. Co-installing up to four backdoors increases resistance (around 36% erased), yet decontaminating a single known co-resident backdoor collaterally clears 52/60 co-residents (87%). Upon visualizing postdecontamination model internals using J-lens, we confirm that although the decontamination restores benign LLM responses, traces of original trigger awareness persist at intermediate layers.

==> sections/3_installation.tex <==
%% ============================================================
\section{Backdoor Installation}
\label{sec:install}
%% ============================================================
% NOTE: merged into 2_framework.tex; no longer \input from the main file.

We first confirm that heterogeneous backdoors install cleanly. Table~\ref{tab:triggers} lists the
validated trigger families and the response menu. A canonical install uses spliced injection
trajectories ($\sim$960 backdoor samples) balanced 1:1 with benign traces, lr~$=3{\times}10^{-5}$
(full) or LoRA rank~16, 1--4 epochs.


\begin{table}[t]
\centering
\label{tab:triggers}
\scriptsize
\setlength{\tabcolsep}{3pt}

\begin{minipage}[t]{0.48\linewidth}
\centering
\begin{tabularx}{\linewidth}{@{}ll>{\raggedright\arraybackslash}X@{}}
\toprule
Type & Trigger & Example value \\
\midrule
\triggerbadge{loccolor}{\trigicon Location}
  & \texttt{reyk/mia/mon}
  & Reykjavik, Miaoli, Montebello \\

\triggerbadge{ipcolor}{\trigicon IP subnet}
  & \texttt{ip2902}
  & 172.29.0.0/16 \\

\triggerbadge{langcolor}{\trigicon Language}
  & \texttt{fr/zh/ja/ar}
  & French, Chinese, Japanese, Arabic \\

\triggerbadge{regcolor}{\trigicon Register}
  & \texttt{formal}
  & formal/bureaucratic \\
\bottomrule
\end{tabularx}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\linewidth}
\centering
\begin{tabularx}{\linewidth}{@{}ll>{\raggedright\arraybackslash}X@{}}
\toprule
Resp. & Suite & Action \\
\midrule
\respcode{dl3}
  & \suitebadge{dailycolor}{DailyLife}
  & delete \texttt{/system/.ssh} \\

\respcode{dl7}
  & \suitebadge{dailycolor}{DailyLife}
  & exfiltrate a file \\

\respcode{dl12}
  & \suitebadge{dailycolor}{DailyLife}
  & create calendar event \\

\respcode{ws1}
  & \suitebadge{workcolor}{Workspace}
  & delete a drive file \\

\respcode{ws14}
  & \suitebadge{workcolor}{Workspace}
  & email an external party \\

\respcode{bk7}
  & \suitebadge{bankcolor}{Banking}
  & change password \\

\respcode{bk9}
  & \suitebadge{bankcolor}{Banking}
  & transfer money \\
\bottomrule
\end{tabularx}
\end{minipage}

\caption{Validated trigger families (left) and the malicious-response menu (right). Each combo installs to $\sim$100\% ASR / 0\% FTR. Recognition phrases let us score recognition independently of execution. System prompt template and associated thought-response in Appendix~\ref{app:vectors}}

\end{table}






A LoRA learning-rate sweep shows installs are clean (ASR~$\geq$95\%, FTR~$<$5\%) but trigger-dependent
in their sensitivity: the language trigger \texttt{fr\_\_dl12} installs at 100\% across
lr~$\in[3{\times}10^{-5},10^{-3}]$, whereas the IP trigger \texttt{ip2902\_\_dl7} reaches only 35\% at
$3{\times}10^{-5}$ and needs lr~$\geq10^{-4}$; at the top of the range FTR becomes leaky. Full per-LR
numbers are in Appendix~\ref{app:results}. Resolved failure modes (data ratio, low-lr phrase
memorization, splicer and thinking-strip bugs) are detailed in Appendix~\ref{app:recipe}.

\paragraph{Installation does not guarantee stealth.} A high ASR does not imply the model still works:
full-weight installs keep benign utility near the base model, but the high-lr LoRA configurations that
reach 100\% ASR \emph{collapse} benign utility to 0--8\% in 6 models (Appendix~\ref{app:results}). An
attacker tuning only for attack success can thus produce an obviously broken agent; stealth is a
separately violable property, which the per-model utility column makes visible.

\FloatBarrier
